Characterizing 1-Dof Henneberg-I graphs with efficient configuration spaces

We define and study exact, efficient representations of realization spaces of a natural class of underconstrained 2D Euclidean Distance Constraint Systems(EDCS) or Frameworks based on 1-dof Henneberg-I graphs. Each representation corresponds to a choice of parameters and yields a different parametrized configuration space. Our notion of efficiency is based on the algebraic complexities of sampling the configuration space and of obtaining a realization from the sample (parametrized) configuration. Significantly, we give purely combinatorial characterizations that capture (i) the class of graphs that have efficient configuration spaces and (ii) the possible choices of representation parameters that yield efficient configuration spaces for a given graph. Our results automatically yield an efficient algorithm for sampling realizations, without missing extreme or boundary realizations. In addition, our results formally show that our definition of efficient configuration space is robust and that our characterizations are tight. We choose the class of 1-dof Henneberg-I graphs in order to take the next step in a systematic and graded program of combinatorial characterizations of efficient configuration spaces. In particular, the results presented here are the first characterizations that go beyond graphs that have connected and convex configuration spaces.

==> contrib.tex <==
%\section{Questions and Contributions}
%\label{sec:contribution}
%
%Here we list 2 natural questions about efficient configuration
%spaces together with the contribution of this manuscript towards answering them.
%
%\subsection{Question 1: Graphs with efficient configuration spaces}
%
%Characterize graphs $G$ for which there is a set $F$ of non-edges such that
%{\sl for all} distance assignments $\delta$ 
%the configuration space $\Phi_F^d(G,\delta)$
%is efficient.
%


These graphs are obtained by deleting a natural {\em base}
edge $f$ from graphs constructed one vertex at a time using a 
natural and commonly used 
{\em Henneberg-I} rule \cite{bib:Laman70}. We call them {\em Simple 
1-dof Henneberg-I graphs} (formally defined in Section \ref{subsec:1dofHen1}).


For this class of graphs $G$, 
we first observe that the natural choice of configuration space 
parameter is the base edge $f$ that has been deleted, i.e, the {\em base non-edge}.
This choice yields the optimal realization complexity for
obtaining a realization, given a parameterized configuration in 
$\Phi_f^2(G,\delta)$.
Fixing this parameter choice 
reduces the above question to 
when such a configuration space has low sampling complexity since 
the realization problem for Henneberg-I graphs is known to be
easy. 
Specifically, this is a 1-parameter
configuration space,  and hence it consists of a union of intervals. 
The sampling complexity is thus 
the complexity of computing the end points (or boundaries) 
of these intervals,
starting with  the EDCS  $(G,\delta)$ as input. 
Our main contributions to Question 1 at the beginning 
of the section are the following.

\begin{itemize}
\item[(1)]
In order to quantify {\em sampling complexity}
we prove the crucial Theorem \ref{thm:config-space}
that associates a {\sl combinatorial meaning} to the end points of the intervals 
in the configuration space $\Phi_f^2(G,\delta)$ for a Simple 
1-dof Henneberg-I graph $G$ with base non-edge $f$.
Specifically, we show that the end points are associated with configurations
of {\em extreme} graphs obtained from $(G,f)$. 
These are formally defined in Section \ref{subsec:1dofHen1}
are are used prominently in Theorem \ref{thm:config-space}.
The proof of this lemma requires basic algebra and real analysis
and also yields Observation \ref{obs:linear-realization-general} that ensures linear realization
complexity for $\Phi_f^2(G,\delta)$.
\end{itemize}

Based on the combinatorial description of   
the configuration spaces $\Phi_f^2(G,\delta)$ given in Theorem \ref{thm:config-space},  
a natural definition of 
{\em low sampling complexity} is obtained by requiring {\sl all the 
extreme graphs obtained from $(G,f)$}
to belong in a class of graphs called {\rm Tree- or Triangle-decomposable} 
graphs 
whose EDCS $(G,\delta)$ are known \cite{bib:Owen02} to 
have relatively low algebraic complexity of realization. 
Hence the corresponding configurations can be relatively easily obtained.
By Theorem \ref{thm:config-space}, this implies a low complexity for computing
the endpoints of the intervals of 
the 1-parameter configuration space 
$\Phi_f^2(G,\delta)$.


\begin{itemize}
\item[(2)]
Based on the above definition of low sampling complexity, Theorem 
\ref{the:TriangleFreeCase}  gives a surprising and  exact forbidden-minor characterization 
of low sampling complexity 
for a large, natural class of Simple 1-dof Henneberg-I graphs.
Observation \ref{obs:backward} notes that the interval end points 
of the 1 parameter configuration spaces 
of such graphs $G$ can be obtained {\sl directly, without 
realizing} the Triangle-decomposable extreme graphs corresponding to $G$.
This is somewhat counterintuitive for the following reasons:
as mentioned above, the characterization in Theorem \ref{the:TriangleFreeCase} relies on 
the Triangle-decomposablility of all the extreme graphs of $G$; 
additionally, by Theorem \ref{thm:config-space}, the interval 
end points of the configuration space
correspond to configurations of extreme graphs; and this in turn 
was our motivation for equating low sampling complexity with purely
Triangle-decomposable extreme graphs, since their configurations
can be easily obtained.

\item[(3)]
Next, the tightness of Theorem \ref{the:TriangleFreeCase}
is illustrated by Observation \ref{obs:TriangleFreeCounter},
Observation \ref{obs:GeneralTriCounter}
and Observation \ref{obs:onepathcounter},  which gives
several examples of graphs that indicate obstructions to obtaining
forbidden minor characterizations 
when any of the restrictions of Theorem \ref{the:TriangleFreeCase} are removed.
When some of them are removed, 
however,  Theorem \ref{the:chain} gives a characterization
of  more general Simple 1-dof Henneberg graphs with 
low sampling complexity, with Triangle-decomposable extreme graphs.
Observation \ref{obs:one-path-not-direct} however gives examples  from this more general class 
for which it is not posible to use
the direct method of Observation \ref{obs:backward} for obtaining the interval end points  
in the configuration space. 

\end{itemize}


\subsection{Question 2: Parameters
that yield efficient configuration spaces for a given graph}

For  graphs $G$ characterized by Question 1 above, 
we would like to characterize the corresponding sets 
of non-edges $F$ such that for all distance assignments $\delta$, 
the configuration space
$\Phi_F^d(G,\delta)$ is efficient.
In addition, we would like to be able to efficiently compute such $F$'s
given $G$. Sometimes it is more convenient to consider a graph
$H$ and characterize those partitions of the edge set of $H$ into 
a graph $G$ and non-edges $F$
such that $\Phi_F^d(G,\delta)$ is efficient.
Our contribution is the following.

\begin{itemize}
\item[(4)]
We show in Theorem \ref{the:quantifierExchange} that 
for Henneberg-I graphs $H$, all 
possible base edges $f$ 
yield equally efficient(or inefficient) configuration spaces
for the corresponding Simple 1-dof Henneberg-I graph $G$, 
i.e, where $H = G\cup f$.
This is an interesting quantifier exchange theorem.
Besides providing
a characterization of all possible parameters that yield efficient
configuration spaces, 
the theorem illustrates the {\sl robustness} of 
our definition of low sampling complexity.
\end{itemize}


%%%%%%%%%\begin{theorem}
%???????????
%For a Henneberg-I graph $H$, consider each possible base edge $f$ that
%gives a Henneberg construction for $H$.
%Let $H_f$ be the Simple 1-dof Henneberg-I graph with base non-edge $f$.
%Then either $\Phi_f^2(H_f,\delta)$ has low sampling complexity for all
%base edges $f$ of $H$ or 
%for none of them.
%See Figure \ref{F:OnePathCounter}.
%
%?????????
%%%%%%%%%%%\end{theorem}



